Semi-Automated Protocol Disambiguation and Code Generation

For decades, Internet protocols have been specified using natural language. Given the ambiguity inherent in such text, it is not surprising that protocol implementations have long exhibited bugs. In this paper, we apply natural language processing (NLP) to effect semi-automated generation of protocol implementations from specification text. Our system, SAGE, can uncover ambiguous or under-specified sentences in specifications; once these are clarified by the spec author, SAGE can generate protocol code automatically. Using SAGE, we discover 5 instances of ambiguity and 6 instances of under-specification in the ICMP RFC; after clarification, SAGE is able to automatically generate code that interoperates perfectly with Linux implementations. We show that SAGE generalizes to BFD, IGMP, and NTP. We also find that SAGE supports many of the conceptual components found in key protocols, suggesting that, with some additional machinery, SAGE may be able to generalize to TCP and BGP.

==> 0_metadata.tex <==
\ifcameraready
\newcommand{\grantack}[1]{
  \ifthenelse{\equal{#1}{CTA}}{\thanks{Research was sponsored by the Army Research Laboratory and was accomplished under Cooperative Agreement Number W911NF-09-2-0053 (the ARL Network Science CTA). The views and conclusions contained in this document are those of the authors and should not be interpreted as representing the official policies, either expressed or implied, of the Army Research Laboratory or the U.S. Government. The U.S. Government is authorized to reproduce and distribute reprints for Government purposes notwithstanding any copyright notation here on.
    }}{}
  \ifthenelse{\equal{#1}{CRA}}{\thanks{Research reported in this paper was sponsored in part by the Army Research Laboratory under Cooperative Agreement W911NF-17-2-0196. The views and conclusions contained in this document are those of the authors and should not be interpreted as representing the official policies, either expressed or implied, of the Army Research Laboratory or the U.S. Government. The U.S. Government is authorized to reproduce and distribute reprints for Government purposes notwithstanding any copyright notation here on.}}{}    
  \ifthenelse{\equal{#1}{NSFAvail}}{\thanks{This material is based upon work supported by the National Science Foundation under Grant No. 1705086}}{}      
  \ifthenelse{\equal{#1}{CPSSyn}}{\thanks{This material is based upon work supported by the National Science Foundation under Grant No. 1330118 and from a grant from General Motors.}}{}        
  \ifthenelse{\equal{#1}{NeTSLarge}}{\thanks{This material is based upon work supported by the National Science Foundation under Grant No. 1413978}}{}          
  \ifthenelse{\equal{#1}{NeTSSmall}}{\thanks{This material is based upon work supported by the National Science Foundation under Grant No. 1423505}}{}
}


%%% Uncomment one or more of the following
%\grantack{CTA}
%\grantack{CRA}
%\grantack{NSFAvail}
%\grantack{CPSSyn}
%\grantack{NeTSLarge}
%\grantack{NeTSSmall}

\fi

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main"
%%% End:


==> background.tex <==

DO NOT EDIT -- NOT IN USE
\section{Background}
\label{section:background}

We have ample anecdotal evidence that protocol specifications are ambiguous and that this leads to bugs and incompatible behavior in implementations. However, to systematize our understanding of such ambiguity and the problems they cause, we examine the problems that arise through a case study of implementations that were part of a graduate networking course. Through this, we are able to identify the sources of common challenges and use them to scope the problems we will tackle through the course of this paper. Here we begin with an informal notion of both protocol specifications and protocol ambiguity, which we refine through the paper.

\subsection{Case Study}

To better understand the existence of ambiguity in general RFCs, we start from a simple but still-central network protocol, Internet Control Message Protocol (ICMP), which we discuss throughout the paper.
ICMP has been a key Internet protocol since its definition nearly 40 years ago, used by \verb=ping=, \verb=traceroute=, routing, and much more.
Compared to other complex protocols, ICMP sender and receiver behaviors are simple and should be, in theory, easy to interpret from the ICMP spec.
For this kind of simple but long-lasting protocol, one might expect that every aspect of its specification would be well-defined and understood by now, but this is not the case.

\begin{figure}[t]
    \centering
    \includegraphics{figs/course_project_topo.pdf}
    \caption{Network topology used in graduate course project to implement ICMP functions}
    \label{fig:project_topo}
\end{figure}

ICMP was formally specified in RFC 792~\cite{rfc792}.  From the spec, we begin with a simple example of ambiguity, in an echo request and reply message exchange.  ICMP's echo message header contains a \verb=checksum= field, computed as follows:
\begin{quote}
\emph{The checksum is the 16-bit one's complement of the one's complement sum of the ICMP message starting with the ICMP Type.}
\end{quote}
One immediate issue of note is that this description does not explicitly mention the end (e.g., bit/byte position) of the checksum computation.
Can this ambiguity, along with other ambiguities in RFC 792, lead to any implementation issues, or is this text ambiguous but innocuous?

To gain a human understanding of specification ambiguity, we collaborated with a graduate level computer networks course, and analyzed an introductory course project with code submissions from 39 students.
For this course project, students were asked to implement \verb=ping=.
The students used an emulation environment built upon Mininet~\cite{lantz2010network} and end hosts were built-in hosts without customization.
Students only needed to write C/C++ code for the one router in the network topology (Figure~\ref{fig:project_topo}).
The expectation was that students would only need to write about 100 lines of code, a simple task.
Students were expected to use RFC 792 as a guide as any questions arose.

We began testing student implementations by sending pings from a client host to \verb=eth3= on the router, and examined the returned echo reply messages and the client's ability to process them.
We deemed an implementation partially correct if the client host was able to parse the received echo reply packet but read an unreasonable round-trip time.
We deemed an implementation wrong if the end host failed to receive or parse the received packets.
Among all 39 submissions, there were 21 fully correct ($\sim$54\%), 3 partially correct ($\sim$8\%) and 15 wrong implementations ($\sim$38\%); the degree to which student implementations were incorrect was surprising.

Looking deeper into each of the 15 implementation failures, excepting 1 that did not compile, the remaining issues fell into 6 categories (not mutually exclusive).
\tabref{t:error_type} shows the list of error types and the frequency of their occurrence.
\textbf{IP (or ICMP) header related} means the errors are due to matching or operations on one or more IP (or ICMP) header field.
\textbf{Byte order conversion} means the implementation confused network and host byte ordering.
\textbf{Incorrect ICMP payload content} means the implementation generated echo reply messages with incorrect information, such as a corruption of the received echo message.
\textbf{Incorrect ICMP echo reply packet length} means the generated echo reply message has an incorrect length for the ICMP payload.
\textbf{Incorrect checksum or dropped by kernel} means the IP or ICMP checksum is wrongly computed and rejected either by kernel code or the student's code.
For built-in Linux generated echo messages, the ICMP \verb=checksum= needs to cover 64 bytes.
Although not all the errors are ICMP-related, we still observe that over half of the failure cases incorrectly handle the ICMP header, something we expected would be simple to handle.

\begin{table}
  \centering
  \footnotesize
  \begin{tabular}{lr}
  \hline
    \tableh{Error Type} & \tableh{Frequency} \\
    \hline
    IP header related & 57\% \\ % 8 cases
    ICMP header related & 57\% \\ % 8 cases
    Network byte order and host byte order conversion & 29\% \\ % 4 cases
    Incorrect ICMP payload content & 43\% \\ % 6 cases
    Incorrect echo reply packet length & 29\% \\ % 4 cases
    Incorrect checksum or dropped by kernel & 36\% \\ % 5 cases
    \hline
  \end{tabular}
  \caption{Error types of failed cases and their frequency in 14 faulty student ICMP implementations.}
  \label{t:error_type}
  \vskip -1em
\end{table}

Lastly, we wanted to determine 1) if any ambiguity in the RFC would lead to different implementations, and 2) how Linux's \verb=ping= reacts to various implementations.
We began with the aforementioned checksum spec ambiguity.
The skeleton code given to the students provided a two-argument checksum function; its first argument was the checksum start pointer and its second argument was the byte count for the checksum calculation.
Our aim was to confirm that students could calculate the ICMP checksum field with different byte counts.
We summarize 9 different ways to represent the number of bytes for computation in Table~\ref{t:cksum_variety}.
From Table~\ref{t:cksum_variety}, we can see significant variation: some students leveraged outer protocol information; another counted only ICMP's header size; still another relied upon magic constants.
Following this observation, we analyzed which answers are acceptable to the client host by picking a correct implementation and only changing the second argument of the built-in checksum function.
To our surprise, the client host accepted any checksum field value computed with whichever integer number.\barath{I'm not clear on what "whichever integer number" means.}
We not only read the ping outcome, but also recorded the received packet.
Neither \verb=ping= nor \verb=tcpdump= ever report any problem with the received packet.

\begin{table}
  \centering
  \scriptsize
  \begin{tabular}{l}
    \hline
    \tableh{Code representations} \\
    \hline
    \lstinline[style=cpp]!sizeof(struct icmp_t3_hdr)! \\
    \lstinline[style=cpp]!sizeof(icmp_hdr)! \\
    \lstinline[style=cpp]!len - sizeof(ethernet_hdr) - sizeof(ip_hdr)! \\
    \lstinline[style=cpp]!ntohs(ip_hdr->ip_len) - ip_hdr->ip_hl * 4! \\
    \lstinline[style=cpp]!sizeof(ip_hdr)! \\
    \lstinline[style=cpp]!sizeof(icmp_hdr) + 4! \\
    \lstinline[style=cpp]!ntohs(ip_hdr->ip_len) - IP_HDR_LEN! \\
    \lstinline[style=cpp]!htons(ntohs(icmp_hdr->icmp_sum) + 0x0800)! \\
    {\footnotesize some constants e.g. \lstinline[style=cpp]!2! or \lstinline[style=cpp]!8! or \lstinline[style=cpp]!36!} \\
    \hline
  \end{tabular}
  \caption{Various code representations for checksum field computation length.}
  \label{t:cksum_variety}
\end{table}

These findings indicate the extent to which even a simple network protocol can be misimplemented.  Our aim is to understand the connection between specification and implementation, and specifically whether ambiguities in the RFC, if any, could lead to sloppy and/or buggy implementations.

%Thus, we take the first step to systematically discover ambiguities in RFC documents, and disambiguate them.  In the process of ambiguity discovery, we identify the key challenges to solve the problem and share our observations.
%In addition, we extend the work to automate code generation from these natural language protocol specifications.

\subsection{Problem Scope}
Here we explain the challenges and current NLP advances for us to tackle automated analysis of natural language protocol specification.

%\subsubsection{Challenges for General Purpose Texts}
%Building a system to convert general purpose program context into executable codes is barely possible.
%To achieve this task, it means we need to have the texts that satisfy both easy for human to write and easy for machine to read.
%However, reducing the difficulty for human to write means human can write vague and verbose words.
%In addition, increasing the easiness for machine to read means machine can precisely interpret every meaning.
%Moreover, there are other challenges to convert human texts into low level codes.
%%Generating low level executable codes from human-written natural language specifications is overwhelmingly challenging but highly desired.
%For example, we need to differentiate what texts are convertible to codes, and what are unnecessary texts.
%For another example, we need to differentiate whether a sentence is meant to describe task A or task B.
%These challenges make it hard to convert human texts into codes.
%%This kind of task is undoubtedly hard to apply on general purpose natural language texts.

%\subsubsection{General Texts to Domain Specific Texts}

\subsubsection{Advantages of Network Protocol Specifications}
Compared to general English text, network protocol specifications are semi-structured documents that may be amenable to automated conversion from natural language to implementation.
%There are a number of reasons to support the feasibility of automated conversion for a network protocol.
The networking community uses a restricted set of words and operations to describe network behaviors; we refer these words and operations as domain-specific language/knowledge.
It is well known in NLP that the accuracy of parsing domain specific languages would be higher than general purpose language.
Networking has significant and unique jargon which, while arcane, could cause less misinterpretation; such jargon is easier for us to convert systematically and accurately.
In addition, official documents specify all major protocols' behavior thus general knowledge and human context is not needed, unlike general NLP.
%For years, the networking community has put efforts into formally documenting protocols.
%More hardware-based research might look into IEEE standards, and more software-based research might check out Request for Comments (RFC) forms.
%For our purpose, we mostly refer to RFC documents for network protocol implementation details.
%The choice of words in RFCs and the author guidelines should be followed to detail protocol behaviors.
%With these reasons, we are more confident to believe it is achievable to automate conversion from formal network protocol specification to runnable codes.


\subsubsection{Problems with Requests For Comments (RFCs)}
Organized by the Internet Engineering Task Force (IETF), the networking community details protocols in Request for Comments (RFC) documents~\cite{RFC}, written in technical but conversational English.
Among these, some RFCs are officially designated as standards.
%For those non-standard RFCs, they are also commonly used as standards globally.
Ideally, as network protocols must enable communication between two or more entities, such RFCs minimize the potential for disagreement and miscommunication.  
%However, on the other hand, these quasi-standard RFCs also create problems due to vague descriptions of some protocol behaviors.

However, our inspection of hundreds of RFCs was a reminder that they are rife with ambiguity, for a diverse array of reasons.
First, RFCs are frequently written by many domain experts but in natural language, which admits greater expressiveness and thus multiple ways to convey the same concepts.
Second, natural language itself may simple be too ambiguous to describe precise protocol behavior without extremely redundant and/or complex text.
Third, context always matters in prose, and given that no compiler exists for prose, an author cannot easily determine whether a term or concept's definition was omitted or its context assumed.
%Besides, every domain expert may focus on different perspectives to describe a protocol, and description formats vary as well.
These ambiguities in both language and technical protocol behavior could significantly impact how an engineer interprets and implements a protocol, leading to buggy and insecure networked systems.
%By some chance, the implemented codes could turn out to be buggy in networked systems.

\begin{figure}[t]
  \centering
  \resizebox{8.3cm}{!}{\input{figs/protocol_approaches.tex}}
  %\vskip -1em
  \caption{Approaches to specifying and implementing network protocols.}
  \label{fig:protocol-approaches}
  %\vskip -1em
\end{figure}

\subsubsection{Natural Language Ambiguities}
Natural languages can have a wide array of types and severities of ambiguities.
Prior work in NLP research has discovered and classified types of ambiguity (e.g., lexical, syntactic, semantic, etc.)~\cite{rayner1986lexical, kempson1981ambiguity}.
Lexical ambiguity refers to a word that itself contains multiple meanings.
For example, \emph{bat} can be a wooden club or a flying mammal.
Syntactic ambiguity is the ambiguity when a sentence has more than one interpretation due to the sentence structure.
For example, \emph{Alice saw Bob with binoculars} is ambiguous because it is unclear whether Alice or Bob has the binoculars.
Semantic ambiguity occurs when a word, phrase, or sentence has more than one meaning without additional context.
For example, \emph{I saw her duck} is unclear as ``her duck'' could refer to a bird or a motion.
All these ambiguities can contribute to incorrect interpretations.
As differentiation of types of language ambiguities is not the main focus of this paper, we will not explicitly classify ambiguities as we discuss them throughout this paper and will refer to all such ambiguities as natural language ambiguities.

\subsection{Related Work}
Our undertaking spans multiple areas of research, from networked systems to NLP to software verification.

\subsubsection{Natural Language Processing (NLP)}
\textbf{Semantic Parsing and Code Generation.}
Semantic parsing is a fundamental task in natural language processing that aims to transform unstructured text into structured logical forms for subsequent execution~\cite{berant2013semantic}.
For example, to answer the question ``Which team does Frank Hoffman play for?'', a semantic parser generates a structured query ``SELECT TEAM from table where PLAYER=Frank Hoffman'' with SQL Standard Grammar \cite{Date1987AGT}.
A SQL interpreter will later execute this query on a database and give the correct answer ``Toronto Argonauts'' \cite{kamath2018survey}.
Apart from the application in question answering, semantic parsing has also been successful in navigating robots \cite{tellex2011understanding}, understanding instructions \cite{chen2011learning} and playing language games \cite{wang2016learning}.
% \noindent\textbf{Code Generation.}
Research in generating code from natural language requires one step beyond logical forms and aims to output concrete implementations in high-level general-purpose programming languages \cite{ling2016latent}. This problem is usually formulated into syntax-constrained sequence generation \cite{yin-neubig-2017-syntactic, liang2016neural}.
The two topics are closely related to our work since the process of implementing network protocols following natural language specifications in RFCs requires the very same ability to understand and execute instructions.

\noindent\textbf{Pre-trained Language Models.} Recently, high-capacity pre-trained language models \cite{peters2018deep, devlin2018bert, yang2019xlnet, lan2019albert} has greatly advanced machine performance in a variety of NLP tasks, including question answering, natural language inference, text classification, etc. The general practice is to first train a large model on huge corpus with unsupervised learning objectives (\textit{i.e.}, pre-training); then re-use these weights to initialize a task-specific model which is later trained with labeled data (\textit{i.e.}, fine-tuning). Related to our work, such pre-trained models advanced the state-of-the-art in semantic parsing \cite{Zhang2019BroadCoverageSP, Zhang2019AMRPA}.
Recent work \cite{Feng2020CodeBERTAP} also attempts to pre-train on programming language and natural language simultaneously, and achieves state-of-the-art performance in tasks of NL code search and code documentation generation. However, direct code generation using pre-trained language models remains to be explored and such approaches require massive datasets.

\subsubsection{Networked systems}
%\barath{Related work from networking, networked systems, operating systems, distributed systems, embedded systems on: 1) protocol specification, 2) protocol design/spec verification, 3) NLP for bug hunting, log analysis, etc., and 4) formally specifying important protocols}
\noindent\textbf{Protocol Languages / Formal Specification Techniques.}
Numerous protocol languages have been proposed over the years.
A few decades ago, Estelle \cite{budkowski1987introduction} and LOTOS \cite{bolognesi1987introduction} intended to provide formal descriptions for OSI protocol suites.
Although these formal description techniques can provide precise protocol behavioral descriptions, it is hard for people to understand and thus use for specification or implementation.
In addition, Estelle used finite state machine specification to depict how protocols communicate in parallel, passing on the complexity, unreadability, and rigidity of modification to followup work \cite{boussinot1991esterel,sidhu1990formal,von1987methods}.
Other research such as RTAG~\cite{anderson1988automated}, x-kernel~\cite{hutchinson1991x}, Morpheus~\cite{abbott1993language}, and Prolac~\cite{kohler1999readable} gradually improved readability, structure, and performance of protocols, spanning specification and implementation.
However, we find, and the networking community has found through experience, that the readability of English-language specifications is still higher than such protocol languages.
To our knowledge, prior work has not revealed the challenges of using English-language specification of protocols.
%Therefore, we discover a number of challenges of using English-based RFC to automatically generate protocol implementation.

\noindent\textbf{Protocol Analysis.}
Past research \cite{bhargavan2002formal,bishop2005rigorous, bolognesi1987introduction} developed techniques to reason about protocol behaviors in an effort to minimize bugs.
Such techniques used specifications of finite state machines, higher-order logic, or domain-specific languages to verify protocols.
Another thread of work \cite{killian2007life, killian2007mace, lee2012gatling} explored the use of explicit-state model-checkerers to find bugs in protocol implementations.
This thread also inspired work (e.g., \cite{pedrosa2015analyzing}) to discover non-interoperabilities in protocol implementations.
%Our work shares the similarity of conducting protocol implementation analysis.
While our aims are similar, our focus is end-to-end, from specification to implementation, and on identifying where ambiguity in specifications leads to bugs.
%However, we focus more in terms of the ambiguity coming from specification and discover the implicit protocol behaviors.

\noindent\textbf{NLP for Log Mining and Parsing.}
Log mining and log parsing are techniques that leverages log files to discover and classify different system events (e.g., 'information', 'warning', and 'error').
Past studies have explored Principal Component Analysis \cite{xu2009detecting}, rule-based analysis \cite{fu2009execution}, statistic analysis \cite{nagaraj2012structured, vaarandi2003data}, and ML-based methods \cite{sipos2014log} to solve log analysis problems.
Recent work \cite{aussel2018improving, bertero2017experience} has applied NLP-based techniques to extract semantic meanings from log files so that event categorization can be improved.
%while we our approach of leveraging NLP mechanisms to classify implementation roles (e.g., sender and receiver) are similar to how these classify log descriptions, their focus  
Their focus is to use semantic parsing of voluminous log output to predict failure events whereas our focus is to use it to generate executable code.

%\jane{I still add the paragraph of program synthesis. I do not know if we are removing this area's related work when we focus more on disambiguation aspect}
\noindent\textbf{Program Synthesis.}
To automatically generate code, prior work explored a range of techniques for program synthesis.
Reactive synthesis \cite{pnueli1989synthesis, piterman2006synthesis} relies on interaction with users to read input for generating output programs.
Inductive synthesis \cite{alur2014syntax} recursively learns logic or functions with incomplete specifications.
Proof-based synthesis (e.g., \cite{srivastava2010program}) takes a correct-by-construction approach to develop inductive proofs to extract programs.
Type-based synthesis \cite{osera2015type, feser2015synthesizing} takes advantage of the types provided from specification to refine output.
In networking community, program synthesis techniques have been applied to automate  (e.g., \cite{mcclurg2015efficient, mcclurg2016event}) the updating of network configurations.
% \jane{LEAVE FOR QINYUAN}
%These ambiguity categories have been discussed under various contexts, but the contexts usually focus on general-purpose need.
%It is relatively unclear how these ambiguities would be identified in domain-specific contexts.
%Especially, ambiguity has barely been pointed out in quasi-standard networking protocol specifications written in natural language.
%In this work, we give some guidance with explanations on how to identify ambiguity systematically.

%\subsubsection{Impact to NLP Community}
%Another potential impact may happen to Natural language processing (NLP) community.
%NLP area puts tons of efforts in solving and understanding general-purpose natural language descriptions.
%Till recent, NLP tools are mature enough to process, analyze and reduce ambiguous in many textual descriptions.
%However, it has been a long period that NLP community puts less focus on domain specific contexts.
%It is unclear how useful these state-of-the-art techniques are towards networking areas.
%Based on the experience in this work, we could identify a number of challenges that NLP community may assist more.

%\subsubsection{General Impact}
%many different directions of studies.
%One direction could be impacting protocol anomaly research.
%Protocol anomaly has been a challenging issue for network community to solve.
%To address the issue, past efforts focus from many aspects including protocol design, protocol validation, protocol verification etc.
%These lines of works focus mostly on the problems after a protocol is already implemented as executable codes.
%Following these lines of work, we might intuitively believe that the long-standing protocols should be robust enough because a great number of studies should have been conducted.
%Therefore, these long-standing protocols should have no troubles in deployment and execution at all.
%However, one can still observe many troubles when a network operates a simple and long-existing protocol.
%Inspired by this, We revisit the question: How can we still make mistakes to deploy a simple protocol?
%There is one critical reason that often gets overseen.
%For any protocol to get deployed universally, a protocol would, at some point, be implemented by an engineer who is not the creator of the protocol.
%Due to lack of deep understanding of a protocol, an engineer must implement the protocol with support of some media.
%One of the most common media is human's natural language descriptions.
%Although network protocol specifications are already much less ambiguous than general texts, any human's natural language could still exist a certain level of ambiguity.
%In this work, we also want to point out the ambiguities that are discovered systematically.
%Furthermore, this work can suggest how a network specification could be more precisely self-explained.

%%The impact of ambiguity in specifications can propagate to network behaviors. A system is needed to fix the problem by automatically discovering and resolving language ambiguity in networking protocol specifications.

%%An unambiguous natural language description in a network protocol specification is necessary to build a robust network. Nonetheless, a robust network not only relies upon unambiguous natural language descriptions but also explicit definitions of protocol behavior. For example, a communication protocol specification could specify different parameters at the sender side, but only address how to handle a subset of parameters at the receiver side. This ambiguity of how to handle the other parameters are not easily discovered. Manual identification of implicit protocol behavior is extremely challenging. One potential solution is to leverage program synthesis techniques to automatically generate code-level implementation of networking protocols and furthermore leverage protocol verification and validation techniques to justify whether the protocol implementation has logical issues.

%\subsection{Challenges}
%\subsubsection{Integrate current NLP tools}
%From our conversation with NLP experts, we learned many NLP tools are sentence-based and are highly impacted by the context. Given a random document, we need to compare if all RFCs share similar document structures. With proper identification of document structure, we could apply sentence-based NLP tools to extract information and analyze language ambiguity. Yet, the document structure can be completely different due to different description styles by different domain experts. We also considered Machine-Learning-based NLP tool as options. However, the challenge is that we have little label data and relatively few protocol specifications (~hundreds), compared to most ML datasets.

%\subsubsection{Choose target protocols}
%There are hundreds of common protocols used in today’s networks. We need to consider both from a language ambiguity perspective and also from an implicit protocol-behavior perspective. To better understand ambiguity, we need to survey the protocols that are well-defined and standing the test of time, so that the human’s intervention to verify the ambiguity and compare protocol behavior could be greatly reduced. Finding a candidate protocol is challenging because many protocols are still implicitly evolving

%\subsubsection{Ambiguity Resolution}
%For an unambiguous protocol description, we mean a description can map to one and only one protocol behavior. We do not mean to rule out the possibility of using another description to describe the identical behavior. However, there is no standard of what should be the format to represent a behavior. In practical, we will need to decide a certain style of intermediate representation to demonstrate a correct protocol behavior.

%\subsubsection{Characteristic of Comparison Metric for Natural Language Ambiguity}
%Generally speaking, when we consider a natural language sentence is more ambiguous compared to unambiguous one, we will describe the ambiguous sentence has more ways of interpretations quantitatively.
%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main"
%%% End:


==> figs/check_eval_igmp.tex <==
\pgfplotsset{
  CheckResultGroup/.style = {
    group/group size = 2 by 1,
    group/vertical sep = 16pt,
    width = .25\textwidth,
    height = .25\textwidth,
    major tick length = 1.5,
    minor tick length = 1,
    tick pos = left,
    yticklabel style = { font = \scriptsize },
    xticklabel style = { font = \scriptsize },
    xlabel near ticks,
    ylabel near ticks,
    legend columns = 4,
    legend cell align = left,
    legend image post style = {yscale=.75, xscale = .3},
    legend style = {
      font = \scriptsize,
      at = {(-.25, 1.1)},
      anchor = south,
      /tikz/every odd column/.append style = {yshift = .75pt},
      /tikz/every even column/.append style = {column sep = 1.5mm},
    },
  },
  CheckPlot/.style = {
    ybar,
    area legend,
    bar width = 10pt,
    xlabel = \empty,
    xtick = \empty,
    symbolic x coords = {Type, ArgOrder, PredOrder, Distributivity},
    enlarge x limits = 1,
    nodes near coords,
    every node near coord/.append style={font=\tiny},
    ylabel style = { font = \scriptsize },
    ylabel shift = -2pt,
  },
  Type/.style = {
    orange,
    fill = orange,
    text = black,
    text opacity = 1,
    error bars/.cd,
    y dir = both,
    y explicit,
  },
  ArgOrder/.style = {
    cyan,
    fill = cyan,
    text = black,
    text opacity = 1,
    error bars/.cd,
    y dir = both,
    y explicit,
  },
  PredOrder/.style = {
    purple,
    fill = purple,
    text = black,
    text opacity = 1,
    error bars/.cd,
    y dir = both,
    y explicit,
  },
  Distributivity/.style = {
    olive,
    fill = olive,
    text = black,
    text opacity = 1,
    error bars/.cd,
    y dir = both,
    y explicit,
  },
}


\begin{tikzpicture}[scale=1]
  %\selectcolormodel{gray}

  \begin{groupplot}[CheckResultGroup]

    \nextgroupplot[
    CheckPlot,
    ylabel = {\# of LFs per Sentence},
    ymin = 0,
    ymax = 1.6,
    ytick = {.5, 1, 1.5},
    minor ytick = {.25, .5, ..., 1.5},
    ]
    \addplot[Type] coordinates { (Type, 0.6) +- (0, 0.6) };
    \addplot[ArgOrder] coordinates { (ArgOrder, 0.6) +- (0, 0.6) };
    \addplot[PredOrder] coordinates { (PredOrder, 0.4) +- (0, 0.4) };
    \addplot[Distributivity] coordinates { (Distributivity, 0.6) +- (0, 0.6) };

    \nextgroupplot[
    CheckPlot,
    ylabel={\# of Affected Sentences},
    ymax = 1.75,
    ymin = 0,
    ytick = {1},
    %minor ytick = {5, 6, ..., 18},
    ]
    \addplot[Type] coordinates { (Type, 1) };
    \addplot[ArgOrder] coordinates { (ArgOrder, 1) };
    \addplot[PredOrder] coordinates { (PredOrder, 1) };
    \addplot[Distributivity] coordinates { (Distributivity, 1) };

    \addlegendimage{Type};
    \addlegendentry{Type};
    \addlegendimage{ArgOrder};
    \addlegendentry{Argument Ordering};
    \addlegendimage{PredOrder};
    \addlegendentry{Predicate Ordering};
    \addlegendimage{Distributivity};
    \addlegendentry{Distributivity};

  \end{groupplot}

\end{tikzpicture}

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../main"
%%% End:


==> figs/checks_common.tex <==
\pgfplotsset{
  EchoChecksPlot/.style = {
    width = .4\textwidth,
    height = .2\textwidth,
    symbolic x coords = {Base, Type, Argument Ordering, Predicate Ordering, Distributivity, Associativity},
    enlarge x limits={upper, value=0.06},
    major tick length = 2,
    minor tick length = 1,
    tick pos = left,
    xticklabels = {, Base, Type, Arg. Order, Pred. Order, Distrib., Assoc.},
    yticklabel style = { font = \scriptsize },
    xticklabel style = { font = \tiny, text width = 1cm, align = center },
    ylabel shift = -2pt,
    xlabel near ticks,
    ylabel near ticks,
    legend cell align = left,
    legend image post style = { scale=0.75 },
    legend style = {
      font = \scriptsize,
      xshift = 1.5pt,
      inner sep = 0.75pt,
      row sep=-1pt,
    },
    legend image code/.code={  % make lines in legend images shorter
      \draw[mark repeat=2,mark phase=2, yshift=1pt]
      plot coordinates {
        (0cm,0cm)
        (0.2cm,0cm)        %% default is (0.3cm,0cm)
        (0.4cm,0cm)         %% default is (0.6cm,0cm)
      };%
    }
  },
  Marker/.style = {
    forget plot,
    mark = *,
    mark options = {solid},
    mark size = 1.75pt,
  },
  Avg/.style = {
    name path = avg,
    black,
    thick,
    Marker,
  },
  Min/.style = {
    name path = min,
    cyan,
    dotted,
    thick,
    Marker,
    mark size = 1.25pt,
  },
  Max/.style = {
    name path = max,
    red,
    dotted,
    thick,
    Marker,
    mark size = 1.25pt,
  },
}


==> figs/lf-graphs-ifcodezero.tex <==
\tikzset{%
  graphnode/.style = {
    draw,
    ellipse,
  },
  graphedge/.style = {
    ->,
  },
  graphtitle/.style = {
    font=\large\bfseries
  },
}

\def\lfgZero {
  \node ('@Condition'1) at (192.5bp,378.0bp) [graphnode] {'@Condition'};
  \node ('@Is'4) at (136.5bp,306.0bp) [graphnode] {'@Is'};
  \node ('@Is'10) at (249.5bp,306.0bp) [graphnode] {'@Is'};
  \node ('Code'6) at (45.5bp,234.0bp) [graphnode] {'Code'};
  \node ('0'7) at (136.5bp,234.0bp) [graphnode] {'0'};
  \node ('@Action'13) at (249.5bp,234.0bp) [graphnode] {'@Action'};
  \node ('0'29) at (367.5bp,234.0bp) [graphnode] {'0'};
  \node ('aid'15) at (122.5bp,162.0bp) [graphnode] {'aid'};
  \node ('@Action'17) at (249.5bp,162.0bp) [graphnode] {'@Action'};
  \node ('identifier'27) at (404.5bp,162.0bp) [graphnode] {'identifier'};
  \node ('match'19) at (184.5bp,90.0bp) [graphnode] {'match'};
  \node ('@And'21) at (314.5bp,90.0bp) [graphnode] {'@And'};
  \node ('Reply'23) at (239.5bp,18.0bp) [graphnode] {'Reply'};
  \node ('timestamp'24) at (389.5bp,18.0bp) [graphnode] {'timestamp'};
  \draw [graphedge] ('@Condition'1) -- ('@Is'4);
  \draw [graphedge] ('@Condition'1) -- ('@Is'10);
  \draw [graphedge] ('@Is'4) -- ('Code'6);
  \draw [graphedge] ('@Is'4) -- ('0'7);
  \draw [graphedge] ('@Is'10) -- ('@Action'13);
  \draw [graphedge] ('@Is'10) -- ('0'29);
  \draw [graphedge] ('@Action'13) -- ('aid'15);
  \draw [graphedge] ('@Action'13) -- ('@Action'17);
  \draw [graphedge] ('@Action'13) -- ('identifier'27);
  \draw [graphedge] ('@Action'17) -- ('match'19);
  \draw [graphedge] ('@Action'17) -- ('@And'21);
  \draw [graphedge] ('@And'21) -- ('Reply'23);
  \draw [graphedge] ('@And'21) -- ('timestamp'24);
}

\def\lfgOne {
  \node ('@Condition'1) at (319.75bp,378.0bp) [graphnode] {'@Condition'};
  \node ('@Is'4) at (268.75bp,306.0bp) [graphnode] {'@Is'};
  \node ('@Is'26) at (371.75bp,306.0bp) [graphnode] {'@Is'};
  \node ('@Action'7) at (156.75bp,234.0bp) [graphnode] {'@Action'};
  \node ('0'23) at (268.75bp,234.0bp) [graphnode] {'0'};
  \node ('Code'28) at (371.75bp,234.0bp) [graphnode] {'Code'};
  \node ('0'29) at (474.75bp,234.0bp) [graphnode] {'0'};
  \node ('aid'9) at (35.747bp,162.0bp) [graphnode] {'aid'};
  \node ('@Action'11) at (156.75bp,162.0bp) [graphnode] {'@Action'};
  \node ('identifier'21) at (311.75bp,162.0bp) [graphnode] {'identifier'};
  \node ('match'13) at (91.747bp,90.0bp) [graphnode] {'match'};
  \node ('@And'15) at (221.75bp,90.0bp) [graphnode] {'@And'};
  \node ('Reply'17) at (146.75bp,18.0bp) [graphnode] {'Reply'};
  \node ('timestamp'18) at (296.75bp,18.0bp) [graphnode] {'timestamp'};
  \draw [graphedge] ('@Condition'1) -- ('@Is'4);
  \draw [graphedge] ('@Condition'1) -- ('@Is'26);
  \draw [graphedge] ('@Is'4) -- ('@Action'7);
  \draw [graphedge] ('@Is'4) -- ('0'23);
  \draw [graphedge] ('@Is'26) -- ('Code'28);
  \draw [graphedge] ('@Is'26) -- ('0'29);
  \draw [graphedge] ('@Action'7) -- ('aid'9);
  \draw [graphedge] ('@Action'7) -- ('@Action'11);
  \draw [graphedge] ('@Action'7) -- ('identifier'21);
  \draw [graphedge] ('@Action'11) -- ('match'13);
  \draw [graphedge] ('@Action'11) -- ('@And'15);
  \draw [graphedge] ('@And'15) -- ('Reply'17);
  \draw [graphedge] ('@And'15) -- ('timestamp'18);
}

\def\lfgTwo {
  \node ('@Condition'1) at (192.5bp,378.0bp) [graphnode] {'@Condition'};
  \node ('@Is'4) at (136.5bp,306.0bp) [graphnode] {'@Is'};
  \node ('@Is'10) at (249.5bp,306.0bp) [graphnode] {'@Is'};
  \node ('Code'6) at (45.5bp,234.0bp) [graphnode] {'Code'};
  \node ('0'7) at (136.5bp,234.0bp) [graphnode] {'0'};
  \node ('@Action'13) at (249.5bp,234.0bp) [graphnode] {'@Action'};
  \node ('0'29) at (367.5bp,234.0bp) [graphnode] {'0'};
  \node ('aid'15) at (134.5bp,162.0bp) [graphnode] {'aid'};
  \node ('@And'17) at (249.5bp,162.0bp) [graphnode] {'@And'};
  \node ('identifier'27) at (392.5bp,162.0bp) [graphnode] {'identifier'};
  \node ('Reply'19) at (179.5bp,90.0bp) [graphnode] {'Reply'};
  \node ('@Action'21) at (318.5bp,90.0bp) [graphnode] {'@Action'};
  \node ('match'23) at (242.5bp,18.0bp) [graphnode] {'match'};
  \node ('timestamp'24) at (394.5bp,18.0bp) [graphnode] {'timestamp'};
  \draw [graphedge] ('@Condition'1) -- ('@Is'4);
  \draw [graphedge] ('@Condition'1) -- ('@Is'10);
  \draw [graphedge] ('@Is'4) -- ('Code'6);
  \draw [graphedge] ('@Is'4) -- ('0'7);
  \draw [graphedge] ('@Is'10) -- ('@Action'13);
  \draw [graphedge] ('@Is'10) -- ('0'29);
  \draw [graphedge] ('@Action'13) -- ('aid'15);
  \draw [graphedge] ('@Action'13) -- ('@And'17);
  \draw [graphedge] ('@Action'13) -- ('identifier'27);
  \draw [graphedge] ('@And'17) -- ('Reply'19);
  \draw [graphedge] ('@And'17) -- ('@Action'21);
  \draw [graphedge] ('@Action'21) -- ('match'23);
  \draw [graphedge] ('@Action'21) -- ('timestamp'24);
}

\def\lfgThree {
  \node ('@Condition'1) at (186.5bp,378.0bp) [graphnode] {'@Condition'};
  \node ('@Is'4) at (135.5bp,306.0bp) [graphnode] {'@Is'};
  \node ('@Is'10) at (238.5bp,306.0bp) [graphnode] {'@Is'};
  \node ('Code'6) at (45.5bp,234.0bp) [graphnode] {'Code'};
  \node ('0'7) at (136.5bp,234.0bp) [graphnode] {'0'};
  \node ('@And'13) at (238.5bp,234.0bp) [graphnode] {'@And'};
  \node ('0'29) at (344.5bp,234.0bp) [graphnode] {'0'};
  \node ('Reply'15) at (168.5bp,162.0bp) [graphnode] {'Reply'};
  \node ('@Action'17) at (307.5bp,162.0bp) [graphnode] {'@Action'};
  \node ('aid'19) at (180.5bp,90.0bp) [graphnode] {'aid'};
  \node ('@Action'21) at (307.5bp,90.0bp) [graphnode] {'@Action'};
  \node ('identifier'26) at (462.5bp,90.0bp) [graphnode] {'identifier'};
  \node ('match'23) at (231.5bp,18.0bp) [graphnode] {'match'};
  \node ('timestamp'24) at (383.5bp,18.0bp) [graphnode] {'timestamp'};
  \draw [graphedge] ('@Condition'1) -- ('@Is'4);
  \draw [graphedge] ('@Condition'1) -- ('@Is'10);
  \draw [graphedge] ('@Is'4) -- ('Code'6);
  \draw [graphedge] ('@Is'4) -- ('0'7);
  \draw [graphedge] ('@Is'10) -- ('@And'13);
  \draw [graphedge] ('@Is'10) -- ('0'29);
  \draw [graphedge] ('@And'13) -- ('Reply'15);
  \draw [graphedge] ('@And'13) -- ('@Action'17);
  \draw [graphedge] ('@Action'17) -- ('aid'19);
  \draw [graphedge] ('@Action'17) -- ('@Action'21);
  \draw [graphedge] ('@Action'17) -- ('identifier'26);
  \draw [graphedge] ('@Action'21) -- ('match'23);
  \draw [graphedge] ('@Action'21) -- ('timestamp'24);
}

\def\lfgFour {
  \node ('@Condition'1) at (307.75bp,378.0bp) [graphnode] {'@Condition'};
  \node ('@Is'4) at (256.75bp,306.0bp) [graphnode] {'@Is'};
  \node ('@Is'26) at (359.75bp,306.0bp) [graphnode] {'@Is'};
  \node ('@Action'7) at (144.75bp,234.0bp) [graphnode] {'@Action'};
  \node ('0'23) at (256.75bp,234.0bp) [graphnode] {'0'};
  \node ('Code'28) at (359.75bp,234.0bp) [graphnode] {'Code'};
  \node ('0'29) at (462.75bp,234.0bp) [graphnode] {'0'};
  \node ('aid'9) at (35.747bp,162.0bp) [graphnode] {'aid'};
  \node ('@And'11) at (144.75bp,162.0bp) [graphnode] {'@And'};
  \node ('identifier'21) at (287.75bp,162.0bp) [graphnode] {'identifier'};
  \node ('Reply'13) at (75.747bp,90.0bp) [graphnode] {'Reply'};
  \node ('@Action'15) at (214.75bp,90.0bp) [graphnode] {'@Action'};
  \node ('match'17) at (138.75bp,18.0bp) [graphnode] {'match'};
  \node ('timestamp'18) at (290.75bp,18.0bp) [graphnode] {'timestamp'};
  \draw [graphedge] ('@Condition'1) -- ('@Is'4);
  \draw [graphedge] ('@Condition'1) -- ('@Is'26);
  \draw [graphedge] ('@Is'4) -- ('@Action'7);
  \draw [graphedge] ('@Is'4) -- ('0'23);
  \draw [graphedge] ('@Is'26) -- ('Code'28);
  \draw [graphedge] ('@Is'26) -- ('0'29);
  \draw [graphedge] ('@Action'7) -- ('aid'9);
  \draw [graphedge] ('@Action'7) -- ('@And'11);
  \draw [graphedge] ('@Action'7) -- ('identifier'21);
  \draw [graphedge] ('@And'11) -- ('Reply'13);
  \draw [graphedge] ('@And'11) -- ('@Action'15);
  \draw [graphedge] ('@Action'15) -- ('match'17);
  \draw [graphedge] ('@Action'15) -- ('timestamp'18);
}

\def\lfgFive {
  \node ('@Condition'1) at (266.1bp,378.0bp) [graphnode] {'@Condition'};
  \node ('@Is'4) at (215.1bp,306.0bp) [graphnode] {'@Is'};
  \node ('@Is'26) at (318.1bp,306.0bp) [graphnode] {'@Is'};
  \node ('@And'7) at (114.1bp,234.0bp) [graphnode] {'@And'};
  \node ('0'23) at (215.1bp,234.0bp) [graphnode] {'0'};
  \node ('Code'28) at (318.1bp,234.0bp) [graphnode] {'Code'};
  \node ('0'29) at (421.1bp,234.0bp) [graphnode] {'0'};
  \node ('Reply'9) at (48.096bp,162.0bp) [graphnode] {'Reply'};
  \node ('@Action'11) at (181.1bp,162.0bp) [graphnode] {'@Action'};
  \node ('aid'13) at (54.096bp,90.0bp) [graphnode] {'aid'};
  \node ('@Action'15) at (181.1bp,90.0bp) [graphnode] {'@Action'};
  \node ('identifier'20) at (336.1bp,90.0bp) [graphnode] {'identifier'};
  \node ('match'17) at (105.1bp,18.0bp) [graphnode] {'match'};
  \node ('timestamp'18) at (257.1bp,18.0bp) [graphnode] {'timestamp'};
  \draw [graphedge] ('@Condition'1) -- ('@Is'4);
  \draw [graphedge] ('@Condition'1) -- ('@Is'26);
  \draw [graphedge] ('@Is'4) -- ('@And'7);
  \draw [graphedge] ('@Is'4) -- ('0'23);
  \draw [graphedge] ('@Is'26) -- ('Code'28);
  \draw [graphedge] ('@Is'26) -- ('0'29);
  \draw [graphedge] ('@And'7) -- ('Reply'9);
  \draw [graphedge] ('@And'7) -- ('@Action'11);
  \draw [graphedge] ('@Action'11) -- ('aid'13);
  \draw [graphedge] ('@Action'11) -- ('@Action'15);
  \draw [graphedge] ('@Action'11) -- ('identifier'20);
  \draw [graphedge] ('@Action'15) -- ('match'17);
  \draw [graphedge] ('@Action'15) -- ('timestamp'18);
}

\begin{tikzpicture}[>=latex,line join=bevel,]

  \matrix[column sep = 10, row sep = -20] {
    %% \node[graphtitle] {LF 0:}; &
    %% \node[graphtitle] {LF 1:}; &
    \node[graphtitle] {LF 2:}; &
    \node[graphtitle] {LF 3:}; &
    \node[graphtitle] {LF 4:}; &
    \node[graphtitle] {LF 5:}; \\

    %% \lfgZero &
    %% \lfgOne &
    \lfgTwo &
    \lfgThree &
    \lfgFour &
    \lfgFive \\
};

\end{tikzpicture}

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../main"
%%% End:

